Programmable Quantum Processors: Equivalence and Learning

In the first part of the work, the equivalence of quantum deterministic and probabilistic processors was investigated. A programmable quantum processor is a device able to transform input data states in a desired way. Deterministic equivalence as well as three types of probabilistic equivalences - strong, weak, and structural - were defined. Necessary and sufficient conditions for deterministic and structural equivalence of unitarily related processors were discovered. Equivalence of deterministic SWAP processor for two-dimensional data and two-dimensional program space was completely solved. It was found that spans of operators of structurally equivalent processors are identical. Relations between types of individual equivalences were also examined. In the second part, robustness of probabilistic storing and retrieval device (PSAR), originally optimized for implementing a phase gate, to noise was examined - specifically to depolarization and phase damping. In the case of a depolarizing channel mixed with a unitary channel, the device implements noisy channel with the probability that decreases with an increasing number of times the given channel is applied. In the case of the phase damping channel, the device implements noisy channel with the same probability as the original PSAR device optimized for phase gate. Concrete implementations - through the Vidal-Masanes-Cirac scheme and virtual qudit - were examined. Vidal-Masanes-Cirac gives the same result for both noisy channels which is better than the result from PSAR. Implementation through virtual qudit for depolarization yields worse probability of successful measurement than Vidal-Masanes-Cirac. However, it is still better than the probability for PSAR. Probability of successful measurement obtained for phase damping implemented through virtual qudit is the same as for Vidal-Masanes-Cirac and PSAR.

==> dissertation/Quantum_Combs.tex <==
Elementary quantum circuits are well described by POVMs, channels and density matrices. It gets more difficult once one begins to combine these circuits together or even if one examines more complicated circuits. There exist infinite possibilities to order various quantum gates in circuits, to combine them with various measurements and to combine quantum circuits into more complicated quantum networks. Furthermore, one has to take into account that every such network can be probabilistic. This means that optimizing networks for various tasks described by multitude of possible networks seems rather complicated. Therefore, one would like to devise an object or device to simplify optimization problems. Luckily, generalizations of POVMs and quantum channels that allow for easier manipulation of quantum networks, do exist \cite{QuantumCircuitArchitecture, QuantumNetworks:GeneralTheoryAndApplications, TheoreticalFrameworkForQuantumNetworks}. 

This new formalism is used in problems such as quantum channel discrimination \cite{TheoreticalFrameworkForQuantumNetworks}, cloning of unitary transformation \cite{OptimalCloningOfUnitaryTransformation} or quantum learning of unitary transformation \cite{OptimalProbabilisticStorageAndRetrievalOfUnitaryChannels} on which we build further in this thesis.

Quantum combs are higher-order structures that map quantum channels into channels \cite{TheoreticalFrameworkForHigher-orderQuantumTheory}. That means that instead of taking quantum states as input , they take quantum channels as input. Quantum comb describes all physically possible transformations by a given quantum network.

\section{Choi-Jamio\l{}kowski Isomorphism}

Choi-Jamio\l{}kowski isomorphism is at the center of our generalized treatment of quantum networks.

But firstly, we shall examine isomorphism between states and operators. Let ${\cal{L(H)}}$ denote set of linear operators on Hilbert space ${\cal{H}}$ and ${\cal{L(H_{A}, H_{B})}}$ denote linear operator from Hilbert space ${\cal{H_{A}}}$ into Hilbert space ${\cal{H_{B}}}$.

Then, let us have an operator $A \in \cal{L}({\cal{L(H_{A})}}, {\cal{L(H_{B})}})$ and a quantum state $\dket{A} \in {\cal{H_{A}}} \otimes {\cal{H_{B}}}$:
\begin{align*}
	A &= \sum_{n,m} \ket{n}\bra{n}A\ket{m}\bra{m} \\
	\dket{A} &= \sum_{n,m} \ket{n}A\bra{m} \ket{n}\ket{m},
\end{align*}
where $\ket{n}, \ket{m}$ denote orthonormal basis of ${\cal{L(H_{A})}}$ and ${\cal{L(H_{B})}}$ respectively. Then the relation:
\begin{align*}
	\dket{A} = (A \otimes \mathbb{I}_{B})\dket{I},
\end{align*}
where $\mathbb{I}_{B}$ denotes identity on ${\cal{H_{B}}}$ and $\dket{I} = \sum_{n}\ket{n}\ket{n}$ is unnormalized maximally entangled state, defines isomorphism between quantum states and quantum operators.

Because, linear operators on Hilbert space also form Hilbert space, we are able to define more general Choi-Jamio\l{}kowski isomorphism between linear maps (or superoperators) and linear operators.

Let ${\cal{L{(L{(H_{A})})},{(L{(H_{B})})}}}$ denote the set of linear maps from the set of linear operators ${\cal{L{(H_{A})}}}$ to the set of linear operators ${\cal{L{(H_{B})}}}$. Then the one-to-one correspondence between linear maps ${\cal{M}}$ from  ${\cal{L{(L{(H_{A})})},{(L{(H_{B})})}}}$ and linear operators $M_{AB}$ on Hilbert space ${\cal{L{(H_{A})}}} \otimes {\cal{L{(H_{B})}}}$ is given in the following definition:
\begin{definition} 
	Choi-Jamio\l{}kowski Isomorphism
	\\
	Let us have map ${\cal{C}}: {\cal{L{(L{(H_{A})})},{(L{(H_{B})})}}} \rightarrow {\cal{H_{A}}} \otimes {\cal{H_{B}}}$. Then Choi-Jamio\l{}kowski isomorphism is given by  
	\begin{align} \label{choi}
		M_{AB} = {\cal{C}}({\cal{M}}) = ({\cal{M}} \otimes {\cal{I_{A}}})(\ket{I}\bra{I}),
	\end{align}
	where ${\cal{I_{B}}}$ is an identity map on ${\cal{L{H_{A}}}}$ and $M_{AB}$ is called Choi operator of map ${\cal{M}}$.
\end{definition}
Inverse of this correspondence (\ref{choi}) is given by:
\begin{align}\label{inverseChoi}
	{\cal{M}}(X) = \Tr_{B}[(I_{A} \otimes X^T)M_{AB}].
\end{align}
\begin{proof}
	\textcolor{red}{mohol by som tu spočítať ten inverse}
\end{proof}

Quantum channels are completely positive, trace-preserving linear transformations and therefore, we shall look at how these qualities translate into Choi operators.
\begin{lemma}
	Trace-preserving
	\\
	Linear map ${\cal{M}}$ is trace-preserving if and only if for its corresponding Choi operator holds the following equation $\Tr_{B}(M_{BA}) = \mathbb{I}_{A}$.
\end{lemma}
\begin{proof}
	content...
\end{proof}

\begin{lemma}
	Complete Positivity
	\\
	Linear map ${\cal{M}}$ is completely positive if and only if its corresponding Choi operators $M_{BA}$ is positive semidefinite.
\end{lemma}
\begin{proof}
	content...
\end{proof}

And let us also add condition on hermiticity.
\begin{lemma}
	Hermiticity
	\\
	Linear map ${\cal{M}}$ is Hermitian if and only if its corresponding Choi operator $M_{BA}$ is Hermitian.
\end{lemma}
\begin{proof}
	content...
\end{proof}

\subsection{Link Product}





















